In Search of Needles in a 11M Haystack: Recurrent Memory Finds What LLMs Miss

This paper addresses the challenge of processing long documents using generative transformer models. To evaluate different approaches, we introduce BABILong, a new benchmark designed to assess model capabilities in extracting and processing distributed facts within extensive texts. Our evaluation, which includes benchmarks for GPT-4 and RAG, reveals that common methods are effective only for sequences up to $10^4$ elements. In contrast, fine-tuning GPT-2 with recurrent memory augmentations enables it to handle tasks involving up to $11\times 10^6$ elements. This achievement marks a substantial leap, as it is by far the longest input processed by any neural network model to date, demonstrating a significant improvement in the processing capabilities for long sequences.

==> table_q1_all_models.tex <==
\begin{table*}[ht]
\caption{Models performance on QA1 task from the BABILong benchmark with PG19 as source of background text.}
\label{tab:results_qa1qa2}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}llllllllllll@{}}
\toprule
\multirow{2}{*}{Model} & \multicolumn{9}{c}{Accuracy, \%} &  \\
\cmidrule(lr){3-11}
& \#params & @4k & @8k & @16k & @32k & @64k & @128k & @500k & @1M & @10M  \\
\midrule
RMT with GPT-2 & 137M & 100.0 & 99.9 & 100.0 & 100.0 & 99.6 & 99.1 & 96.4 & 94.2 & 81.8 \\
RMT with GPT-2 and self-retrieval & 137M & 99.9 & 99.8 & 99.9 & 99.9 & 99.7 & 99.5 & 97.5 & 97.4 & 86.0 \\
mistral-medium (all documents in the context) & - & 73.0 & 75.0 & 58.0 & 33.0 & & & & & \\
GPT4 (all documents in the context) & - & 97.0 & 93.0 & 66.0 & 43.0 & 30.0 & 24.0 & & & \\
\midrule
GPT4+RAG, sentences, top k=1 & - & & 72.0 & & 60.0 & 62.0 & & 44.0 & \\
GPT4+RAG, sentences, top k=5 & - & & 50.0 & & 50.0 & 60.0 & & 56.0 & \\
GPT4+RAG, 512 tokens, top k=1 & - & & 30.0 & & 14.0 & 8.0 & & 4.0 & \\
GPT4+RAG, 512 tokens, top k=5 & - & & 58.0 & & 24.0 & 16.0 & & 12.0 & \\
\midrule
Retrieval quality, sentences, top k=1 & - & & 70.0 & & 60.0 & 58.0 & & 40.0 & \\
Retrieval quality, sentences, top k=5 & - & & 100.0 & & 94.0 & 98.0 & & 82.0 & \\
Retrieval quality, 512 tokens, top k=1 & - & & 32.0 & & 14.0 & 2.0 & & 4.0 & \\
Retrieval quality, 512 tokens, top k=5 & - & & 76.0 & & 34.0 & 14.0 & & 14.0 & \\
Retrieval quality, wiki, 250 tokens, top k=1 & - & & 29.0 & & 18.0 & 9.0 & 2.0 & 1.0 & 0.0 \\
Retrieval quality, wiki, 250 tokens, top k=5 & - & & 78.0 & & 50.0 & 30.0 & 18.0 & 4.0 & 0.0 \\
\midrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\end{table*}


